Sintel: A Machine Learning Framework to Extract Insights from Signals

The detection of anomalies in time series data is a critical task with many monitoring applications. Existing systems often fail to encompass an end-to-end detection process, to facilitate comparative analysis of various anomaly detection methods, or to incorporate human knowledge to refine output. This precludes current methods from being used in real-world settings by practitioners who are not ML experts. In this paper, we introduce Sintel, a machine learning framework for end-to-end time series tasks such as anomaly detection. The framework uses state-of-the-art approaches to support all steps of the anomaly detection process. Sintel logs the entire anomaly detection journey, providing detailed documentation of anomalies over time. It enables users to analyze signals, compare methods, and investigate anomalies through an interactive visualization tool, where they can annotate, modify, create, and remove events. Using these annotations, the framework leverages human knowledge to improve the anomaly detection pipeline. We demonstrate the usability, efficiency, and effectiveness of Sintel through a series of experiments on three public time series datasets, as well as one real-world use case involving spacecraft experts tasked with anomaly analysis tasks. Sintel's framework, code, and datasets are open-sourced at https://github.com/sintel-dev/.

==> figures/hyperopt.tex <==
\begin{figure}[!t]
\centering
\begin{tikzpicture}[scale=0.9]
%\pgfplotsset{set layers}
\begin{axis}[
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},  
    align = center,
    title style={font=\footnotesize},
    title={Optimization of hyperparameters for the \\ LSTM prediction pipeline on Signal S1},
    axis y line*=left,
    xlabel={Iterations},
    ylabel={F1 Score},
    height=5cm,
    width=\linewidth,
    %xmin=0, xmax=100,
    %ymin=0, 
    ymax=1,
    %xtick={0,20,40,60,80,100},
    %ytick={0,20,40,60,80,100,120},
    %legend pos=north west,
    legend style= {font=\footnotesize, at={(0.36,-0.23)}},
    %ymajorgrids=true,
    %grid style=dashed,
]
 
% \addplot[
%     color=ACMDarkBlue,
%     %mark=square,
%     line width=0.8pt,
%     ]
%     coordinates {
%     (0,0)(1,0)(2,0)(3,0.777)(4,0.756)(5,0.732)(6,0.868)(7,0)(8,0.207)(9,0)(10,0.646)(11,0.178)(12,0)(13,0)(14,0)(15,0.207)(16,0)(17,0.878)(18,0)(19,0)
%     };
%     \addlegendentry{F1 score}
    
\addplot[
    % color=ACMDarkBlue,
    %mark=square,
    line width=0.8pt,
    ]
    coordinates {
    (0,0)(1,0)(2,0)(3,0.777)(4,0.777)(5,0.777)(6,0.868)(7,0.868)(8,0.868)(9,0.868)(10,0.868)(11,0.868)(12,0.868)(13,0.868)(14,0.868)(15,0.868)(16,0.868)(17,0.878)(18,0.878)(19,0.878)
    };
    \addlegendentry{Best F1 score}
    
\end{axis}

\begin{axis}[
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},  
    axis y line*=right, 
    axis x line=none,
    ylabel={Percentage of specified range},
    height=5cm,
    width=\linewidth,
    %xmin=0, xmax=100,
    %ymin=0, ymax=120,
    %xtick={0,20,40,60,80,100},
    %ytick={0,20,40,60,80,100,120},
    %legend pos=north west,
    legend cell align={left},
    legend style= {font=\footnotesize, at={(1,-0.23)}},
    %ymajorgrids=true,
    %grid style=dashed,
]
 
\addplot[
    % color=ACMGreen!40,
    %mark=square,
    line width=0.6pt,
    ]
    coordinates {
    (0,381/5)(1,187/5)(2,437/5)(3,173/5)(4,147/5)(5,116/5)(6,24/5)(7,428/5)(8,483/5)(9,437/5)(10,451/5)(11,302/5)(12,166/5)(13,19/5)(14,400/5)(15,245/5)(16,180/5)(17,247/5)(18,79/5)(19,108/5)
    };
    %\legend{LSTM units 1st layer}
    \addlegendentry{LSTM units 1\textsuperscript{st} layer}

\addplot[
    % color=ACMPurple!40,
    %mark=square,
    line width=0.6pt,
    ]
    coordinates {
    (0,167/5)(1,110/5)(2,495/5)(3,320/5)(4,194/5)(5,310/5)(6,124/5)(7,330/5)(8,249/5)(9,417/5)(10,69/5)(11,90/5)(12,308/5)(13,386/5)(14,88/5)(15,56/5)(16,318/5)(17,469/5)(18,453/5)(19,307/5)
    };
    \addlegendentry{LSTM units 2\textsuperscript{nd} layer}    

\end{axis}
\end{tikzpicture}
\caption{Example showing the hyperparameter optimization for the LSTM units in the first and second layer over a period of 20 iterations and the corresponding F1 score using BTB.} 
\label{fig:hypterparameteroptimization}
\end{figure}

==> listings/automl.tex <==
\newenvironment{algocolor}{%
   \setlength{\parindent}{0pt}
   \itshape
   \color{blue}
}{}

\begin{algorithm}
\begin{algocolor}
\SetKw{KwReturn}{return}
\KwIn{template $T$, dataset $D$, scorer function $f$, budget $B$.}
\KwOut{best hyperparameter $\lambda^\ast$}
%  \vspace{0.2em}
 \SetKwBlock{Begin}{begin}{}
 \SetKwFunction{KwFunction}{cross\_validate}
 \Begin{
  $\texttt{init Tuner}$  \hfill \tcp{Bayesian Tuner from \texttt{BTB}}
  $s^\ast \leftarrow + \infty, \lambda^\ast \leftarrow \varnothing$\;
  \While{$B > 0 \land s^\ast \neq f^\ast$}{
   $\lambda \leftarrow \texttt{Tuner.propose}(T)$ \hfill \tcp{propose a set of hyperparameters}
   $P \leftarrow (T, \lambda)$\;
   $s \leftarrow \KwFunction(f, P, D)$\;
   $\texttt{Tuner.record}(\lambda, s)$ \hfill \tcp{update tuner}
    \If{$s < s^\ast$}{
     $s^\ast \leftarrow s$\;
     $\lambda^\ast \leftarrow \lambda$\;
    }
    {\normalfont reduce($B$)} \hfill \tcp{decrease budget}
  }
 \KwReturn{$\lambda^\ast$}
 }
 \caption{Automated hyperparameter optimization in \sintel, searching for the best configuration of $\lambda$ and evaluating pipelines using the scoring function $f$.}
 \label{algo:automl}
\end{algocolor}
\end{algorithm}
% \vspace{-0.5cm}

==> tables/annotations.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{lcc}
    \toprule
    & ML                  & ML    \\
    & identified          & missed    \\
    \midrule
    Normal          & 56                 & 2                 \\
    Problematic     & 11                 & 6                 \\
    Investigate     & 16                 & 19                 \\
    \midrule
    Total           & 83                 & 27                 \\
    \bottomrule
    \end{tabular}
    \caption{} % \review{In-depth post-analysis of events.}}
    \label{tab:annotations}
\end{table}

==> tables/benchmark_f1_pre_rec_signal.tex <==

 \begin{table*}[!b]
 \caption{Precision, Recall and F1-Scores of pipelines}
 \begin{tabulary}{\textwidth}{*{2}{L}*{11}{c}}
 \toprule
  & & \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo S5} & \multicolumn{5}{c}{NAB}  \\
   \cmidrule(r){3-4}\cmidrule(r){5-8}\cmidrule(r){9-13}
 \textbf{Variation} & & MSL & SMAP & A1 & A2 & A3 & A4 & Art & AWS & AdEx & Traf & Tweets\\
 \midrule
 \multirow{3}{*}{LSTM DT}
 & P    & 0.375 & 0.680 
        & 0.690 & 0.966 & 0.991 & 0.893 
        & 0.333 & 0.391 & 0.625 & 0.542 & 0.538 \\
 & R    & 0.667 & 0.761 
        & 0.815 & 0.985 & 0.589 & 0.510 
        & 0.500 & 0.600 & 0.909 & 0.929 & 0.636 \\
 & F1   & 0.480 & 0.718 
        & 0.747 & 0.975 & 0.739 & 0.649 
        & 0.400 & 0.474 & 0.741 & 0.684 &0.583 \\
 \hline
 \multirow{3}{*}{TadGAN}
 & P    & 0.451 & 0.573 
        & 0.592 & 0.792 & 0.764 & 0.575 
        & 0.625 & 0.625 & 0.625 & 0.391 & 0.559 \\
 & R    & 0.639 & 0.761 
        & 0.522 & 0.855 & 0.358 & 0.280 
        & 0.833 & 0.667 & 0.909 & 0.643 & 0.576 \\
 & F1   & 0.529 & 0.654 
        & 0.555 & 0.822 & 0.487 & 0.377 
        & 0.714 & 0.645 & 0.741 & 0.486 & 0.567 \\
 \hline
 \multirow{3}{*}{LSTM AE} 
 & P    & 0.450 & 0.635 
        & 0.629 & 0.833 & 0.931 & 0.711 
        & 0.667 & 0.840 & 0.533 & 0.412 & 0.640 \\
 & R    & 0.500 & 0.701 
        & 0.562 & 0.900 & 0.286 & 0.171 
        & 0.667 & 0.700 & 0.727 & 0.500 & 0.485 \\
 & F1   & 0.474 & 0.667 
        & 0.593 & 0.865 & 0.438 & 0.276 
        & 0.667 & 0.764 & 0.615 & 0.452 & 0.552 \\
 \hline
 \multirow{3}{*}{ARIMA} 
 & P    & 0.393 & 0.304 
        & 0.684 & 0.772 & 0.998 & 0.955 
        & 0.375 & 0.405 & 0.727 & 0.429 & 0.444 \\
 & R    & 0.306 & 0.313 
        & 0.815 & 0.865 & 0.643 & 0.533 
        & 0.500 & 0.567 & 0.727 & 0.429 & 0.606 \\
 & F1   & 0.344 & 0.309 
        & 0.744 & 0.816 & 0.782 & 0.684 
        & 0.429 & 0.472 & 0.727 & 0.429 & 0.513 \\
 \hline
 \multirow{3}{*}{Dense AE} 
 & P    & 0.567 & 0.712 
        & 0.719 & 0.955 & 0.975 & 0.586 
        & 0.600 & 0.846 & 0.667 & 0.529 & 0.600 \\
 & R    & 0.472 & 0.627 
        & 0.590 & 0.845 & 0.042 & 0.049 
        & 0.500 & 0.733 & 0.545 &  0.643 & 0.455 \\
 & F1   & 0.515 & 0.667 
        & 0.648 & 0.897 & 0.080 & 0.091 
        & 0.545 & 0.786 & 0.600 & 0.581 & 0.517 \\
 \hline
 \multirow{3}{*}{MS Azure} 
 & P    & \\
 & R    & \\
 & F1   & \\
 \bottomrule
 \end{tabulary}
 \label{tab:results_appendix}
 \end{table*}
 
 

==> texfiles/challenges.tex <==
\section{Motivation}

There are many challenges in designing an anomaly detection system at scale.
We illustrate some of the most common problems and how they are motivating the development of our new system.

\paragraph{Challenge 1: Generalization} With different signals comes a variety of anomalies. Existing approaches excel at detecting anomalies in certain behaviors but fail in others. There are many different approaches for anomaly detection, but there is no single pipeline that can solve everyone's problem. Furthermore, each pipeline is composed of a wide range of pre- post-processing methods for time series (e.g., aggregation, normalization, etc.), giving a nearly infinite number of different possible options. Moreover, machine learning is a continuously growing field, we ask ourselves, how can we keep up with the latest and greatest? 

\paragraph{Challenge 2: Cold-start and Lack of Labels} In a typical time series setting, the monitoring application is flooded with thousands of signals. The analyst is left with a daunting question, ``where shall I start?''. It is difficult to expect users to label these signals manually. Some domain knowledge comes into play in this situation, analysts limit their investigations to critical signals and often neglect the other hundred thousand. To successfully build an anomaly detector,  developers should enable the system to process a large number of signals and suggest potential anomalies. Unsupervised learning approaches achieves this expectation by detecting anomalies in situations where we do not have labels and signals are not fixated on a particular pattern.

\paragraph{Challenge 3: Feedback} Providing a set of potential anomalies is only the first part of an anomaly detector. The second part is feeding the annotations of the analyst back into the system. The human-in-the-loop integration is essential for continuous learning. Major systems ignore this aspect of the problem.

\paragraph{Challenge 4: Usability and Interaction} Many of the proposed methods require substantial programming knowledge, or in the case of Machine Learning (ML) based methods, even ML knowledge. In other fields of ML, different systems were proposed to improve the human interaction. For example, \citet{Shang2019} try to achieve a better interaction of domain expertise and statistical knowledge by proposing a new Interactive AutoML tool. Yet, for the area of anomaly detection, which requires a very specific interaction and visualization, we are not aware of any work that addresses this gap. To overcome this hurdle, we design a system that serves three classes of populations.
\begin{enumerate}
    \item \textit{machine learning researchers} that want to access the some of the best anomaly detection methods.
    \item \textit{system developers} that want to build their own anomaly detection system.
    \item \textit{end users} (data analysts) that want to detect anomalies within their own data.
\end{enumerate}

\par

In \textit{Orion}, we address all of these challenges and present a system that (1) is easy to use by anyone; even a non-machine learning expert, by providing a set of coherent APIs; (2) is general for any time series data; (3) unlimited and not constraint by a particular anomaly detection pipeline; (4) pair these pipelines with a sequence hyperameters tunning and model selection strategies~\citep{smith2019machine, Bergstra2012, luo2016review, Binnig2018}; (5) allows for pipeline performance comparison through the benchmarking component;  (6) integrates expert feedback into the system; (7) provides a visualization component for efficient anomaly annotations.

